Statistical Guarantees for Variational Autoencoders using PAC-Bayesian Theory

Since their inception, Variational Autoencoders (VAEs) have become central in machine learning. Despite their widespread use, numerous questions regarding their theoretical properties remain open. Using PAC-Bayesian theory, this work develops statistical guarantees for VAEs. First, we derive the first PAC-Bayesian bound for posterior distributions conditioned on individual samples from the data-generating distribution. Then, we utilize this result to develop generalization guarantees for the VAE's reconstruction loss, as well as upper bounds on the distance between the input and the regenerated distributions. More importantly, we provide upper bounds on the Wasserstein distance between the input distribution and the distribution defined by the VAE's generative model.

==> my-macros.tex <==
\usepackage[final]{neurips_2023}



\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[colorlinks=true, citecolor=blue]{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage[dvipsnames]{xcolor}         % colors
\usepackage{lipsum}
\usepackage{import}
\usepackage{xr}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%   MY MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{hyperref}
\usepackage{graphicx}
\usepackage{bm}

\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environnement deriv pour les derivations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newlength{\indentationFormule} 
\setlength{\indentationFormule}{1.3em}
\newlength{\indentationTotaleFormule}
\newlength{\indentationCommentaire}
\setlength{\indentationCommentaire}{4em}
\newlength{\indentationDerivation}
\newlength{\largeurLangle}
\settowidth{\largeurLangle}{$\langle$\hspace*{.4em}}
\newlength{\largeurBoiteCommentaire}
%\newlength{\predboxwidth}
%\newlength{\savebaselineskip}
%\newlength{\derivationskip}


%\makeatletter
%\newcommand{\@indenteFormule}{\hspace*{\indentationFormule}}
\newenvironment{deriv}[1][\leftmargini]%
{\setlength{\indentationDerivation}{#1}%
\setlength{\indentationTotaleFormule}{\indentationFormule}
\addtolength{\indentationTotaleFormule}{#1}
\setlength{\largeurBoiteCommentaire}{\linewidth}
\addtolength{\largeurBoiteCommentaire}{-\indentationFormule}
\addtolength{\largeurBoiteCommentaire}{-\indentationCommentaire}
\addtolength{\largeurBoiteCommentaire}{-\largeurLangle}
\addtolength{\largeurBoiteCommentaire}{-\indentationDerivation}
\begin{list}{}{\setlength{\leftmargin}{\indentationTotaleFormule}}
\setlength{\baselineskip}{2.3\baselineskip}
\item$}%
{\hbox{}$\end{list}}  % \hbox{} evite des erfull lors d'usages
% sans \< et sans \commentaire (et avec
% des \\ pour changer de ligne).
%    \trivlist\item\relax\let\>\@indenteFormule\leftskip\indentationTotaleFormule$}%
%   {\hbox{}$\endtrivlist}  % \hbox{} evite des underfull lors d'usages sans \< et sans \commentaire.

\newcommand{\<}[1]{\newline \hspace*{-\indentationFormule}\makebox(0,0)[bl]{$#1$}\hspace*{\indentationFormule}}

\newcommand{\commentaire}[1]{\hspace*{\indentationCommentaire}\langle\hspace*{.4em}%
\begin{minipage}[t]{\largeurBoiteCommentaire}%
#1 $\rangle$\\\hbox{}% Bizarre. Pourquoi ea prend \\ ici et aussi e la ligne suivante ?
% Sans \hbox{}, il y a des underfull.
\end{minipage}\\[-1ex] % Sans ces deux \\, l'espace apres un commentaire n'est pas le meme quand
% le commentaire a plus d'une ligne.
}

\newcommand{\commentaireligne}[1]{\mbox{\mm ---#1}}
\newcommand{\sepcom}{\mbox{ }\&\hspace{.3em}\ }



%%%%%%%%%%%%%%%% Emojis and Jokes  %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dunno}[1][]{%
\begin{tikzpicture}[baseline,x=0.8\ht\strutbox,y=0.8\ht\strutbox,line width=0.125ex,#1]
\def\arm{(-2.5,0.95) to (-2,0.95) (-1.9,1) to (-1.5,0) (-1.35,0) to (-0.8,0)};
\draw \arm;
\draw[xscale=-1] \arm;
\def\headpart{(0.6,0) arc[start angle=-40, end angle=40,x radius=0.6,y radius=0.8]};
\draw \headpart;
\draw[xscale=-1] \headpart;
\def\eye{(-0.075,0.15) .. controls (0.02,0) .. (0.075,-0.15)};
\draw[shift={(-0.3,0.8)}] \eye;
\draw[shift={(0,0.85)}] \eye;
% draw mouth
\draw (-0.1,0.2) to [out=15,in=-100] (0.4,0.95); 
\end{tikzpicture}}


\newcommand{\smilyface}{...}
\newcommand{\sadface}{...}




%%%%%%%%%%%%%% Theorems %%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\newtheorem{proposition}[theorem]{Proposition}
\numberwithin{theorem}{section}
\newtheorem{corollary}[theorem]{Corollary}
\numberwithin{theorem}{section}
\newtheorem{lemma}[theorem]{Lemma}
\numberwithin{theorem}{section}

\theoremstyle{definition}
\newtheorem{example}{Example}
\numberwithin{example}{section}
\newtheorem{fact}{FACT}
\numberwithin{fact}{section}
\newtheorem{remark}{Remark}
\numberwithin{remark}{section}
\newtheorem{hypothesis}{Hypothesis}
\numberwithin{hypothesis}{section}
\newtheorem{definition}{Definition}
\numberwithin{definition}{section}
\newtheorem{assumption}{Assumption}





%%%%%%%%%%%%%%%%% Logic Symbols %%%%%%%%%%%%
\newcommand{\vrai}{\ensuremath{\mathsf{vrai}}}
\newcommand {\vr}{\ensuremath{\mathsf{v}}}
\newcommand {\faux}{\ensuremath{\mathsf{faux}}}
\newcommand {\fa}{\ensuremath{\mathsf{f}}}
\newcommand{\non}{\neg}
\newcommand{\et}{\wedge}
\newcommand{\etL}{\,\wedge\,}
\newcommand{\etLL}{\,\,\wedge\,\,}
\newcommand{\ou}{\vee}
\newcommand{\ouL}{\,\vee\,}
\newcommand{\ouLL}{\,\,\vee\,\,}
\newcommand{\ssi}{\Leftrightarrow}
\newcommand{\ssiL}{\,\Leftrightarrow\,}
\newcommand{\ssidef}{\,\stackrel{\mathclap{\mbox{\tiny déf}}}{\ssi}\,}
\newcommand{\ssiLL}{\,\,\Leftrightarrow\,\,}
\newcommand{\imp}{\Rightarrow}
\newcommand{\impL}{\,\Rightarrow\,}
\newcommand{\impLL}{\,\,\Rightarrow\,\,}
\newcommand{\cons}{\Leftarrow}
\newcommand{\consL}{\,\Leftarrow\,}
\newcommand{\consLL}{\,\,\Leftarrow\,\,}






%%%%%%%%%%%%%%%  Quantifiers  %%%%%%%%%%%%%%%%%%
\newcommand{\restrict}[2]{#1_{|#2}}
\newcommand{\somme}[3]{\sum_{#1}^{#2}{#3}}
\newcommand{\produit}[3]{\prod_{#1}^{#2}{#3}}
\newcommand{\integral}[4]{\int_{#1}^{#2} #3 \,#4}
\newcommand{\unionq}[3]{\bigcup_{#1}^{#2}{#3}}
\newcommand{\intersectq}[3]{\bigcap_{#1}^{#2}{#3}}


%%%%%%%%%%%%%%%%  Sets  %%%%%%%%%%%%%%%%%%%%%
\newcommand{\nat}{\mathbb{N}} 
\newcommand{\real}{\mathbb{R}}
\newcommand{\incl}{\subset}
\newcommand{\sphere}[1]{\mathbb{S}^{#1}}
\newcommand{\theset}[1]{\{ #1 \}}
\newcommand{\lipschitz}[1]{\text{\rm Lip}_{#1} }
\newcommand{\power}[1]{\pfancy\left( #1 \right)}



%%%%%%%%%%%%%%%%  Variables  %%%%%%%%%%%%%%%%%%%%
\newcommand{\loss}{\ell}
\newcommand{\xfancy}{\mathcal{X}}
\newcommand{\yfancy}{\mathcal{Y}}
\newcommand{\zfancy}{\mathcal{Z}}
\newcommand{\dfancy}{\mathcal{D}}
\newcommand{\hfancy}{\mathcal{H}}
\newcommand{\lfancy}{\mathcal{L}}
\newcommand{\ffancy}{\mathcal{F}}
\newcommand{\gfancy}{\mathcal{G}}
\newcommand{\tfancy}{\mathcal{T}}
\newcommand{\ufancy}{\mathcal{U}}
\newcommand{\wfancy}{\mathcal{W}}
\newcommand{\pfancy}{\mathcal{P}}
\newcommand{\qfancy}{\mathcal{Q}}
\newcommand{\rfancy}{\mathcal{R}}
\newcommand{\sfancy}{\mathcal{S}}
\newcommand{\kfancy}{\mathcal{K}}
\newcommand{\sigmasq}{\sigvector^2}
\newcommand{\sigmmatrix}{\bm{\Sigma}}
\newcommand{\xmatrix}{\mathbf{X}}
\newcommand{\lammatrix}{\bm{\Lambda}}
\newcommand{\zeromatrix}{\mathbf{0}}
\newcommand{\idmatrix}{\mathbf{I}}
\newcommand{\sigvector}{\bm{\sigma}}
\newcommand{\muvector}{\bm{\mu}}
\newcommand{\zvector}{\mathbf{z}}
\newcommand{\yvector}{\mathbf{y}}
\newcommand{\xvector}{\mathbf{x}}
\newcommand{\cvector}{\mathbf{c}}
\newcommand{\hvector}{\mathbf{h}}
\newcommand{\uvector}{\mathbf{u}}
\newcommand{\wvector}{\mathbf{w}}
\newcommand{\epsvector}{\bm{\epsilon}}
\newcommand{\pivector}{\bm{\pi}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\const}{\text{Const}}
\newcommand{\dimz}{{d_\zfancy}}




%%%%%%%%%%%%%%%%%%%  Operators  %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dotproduct}[2]{\langle #1, #2 \rangle}
\newcommand{\equdef}{\stackrel{\text{def}}{=}}
\newcommand{\sampled}{\sim}
\newcommand{\iidsampled}{\stackrel{\text{iid}}{\sim}}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\absolu}[1]{\left \lvert #1 \right \rvert}
\newcommand{\partderiv}[1]{\frac{\partial}{\partial #1}}
\newcommand{\gradient}[2]{\nabla_{#1}{#2}}





%%%%%%%%%%%%%%%%  Functions  %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\expon}[1]{e^{#1}}
\newcommand{\exponbig}[1]{\textnormal{exp}\left[ #1    \right]}
\newcommand{\argmin}[2]{\underset{#1}{\text{argmin }} #2}
\newcommand{\argmax}[2]{\underset{#1}{\text{argmax }} #2}
\newcommand{\minfunc}[2]{\underset{#1}{\text{min }} #2}
\newcommand{\supremum}[2]{\sup_{#1} #2}
\newcommand{\lipnorm}[1]{\norm{#1}_{\textrm{Lip}}}




%%%%%%%%%%%%%%%%  Probabilities and Statistics %%%%%%%%%%%%%%%
\newcommand{\pushf}[2]{{#1} \sharp #2}
\newcommand{\Coupling}[1]{\Gamma(#1)}
\newcommand{\wasserstein}[2]{\text{W}_{#1}(#2)}
\newcommand{\ipm}[1]{d_{#1}}
\newcommand{\prob}[2]{\underset{#1}{\mathbb{P}}\left[#2\right]}
%\newcommand{\expect}[2]{\underset{#1}{\mathbb{E}}\left[#2\right]}
\DeclareMathOperator*{\Esp}{\mathbb{E}}
\newcommand{\expect}[2]{\Esp_{#1}\left[#2\right]}
\newcommand{\expectseul}[2]{\Esp_{#1} #2 }
\newcommand{\expecttext}[2]{\Esp_{#1}\,[#2]}

\newcommand{\variance}[2]{\underset{#1}{\mathbb{V}} \left[ #2 \right] }
\newcommand{\variancehat}[2]{\underset{#1}{\hat{\mathbb{V}}} \left[ #2 \right] }
\newcommand{\varianceseul}[2]{\underset{#1}{\mathbb{V}} \,#2  }
\newcommand{\normal}[1]{\mathcal{N}(#1)}
\newcommand{\mprob}[1]{\mathcal{M}_+^1(#1)}
\newcommand{\kl}[2]{\mathrm{KL}(#1 \, || \, #2)}
\newcommand{\js}[2]{\mathrm{JS}(#1 \, || \, #2)}
\newcommand{\abscont}{\ll}
\newcommand{\uniform}[1]{\ufancy_{#1}}



%%%%%%%%%%%%%%%%  Formatting &  Miscellaneous  %%%%%%%%%%%%%%%
\newcommand{\listen}[1]{#1_1, \dots, #1_n}
\newcommand{\crochet}[1]{\langle #1 \rangle}
\newcommand{\rouge}[1]{\textcolor{red}{#1}}
\newcommand{\bleu}[1]{\textcolor{blue}{#1}}
\newcommand{\details}[1]{\bleu{#1}}
\newcommand{\askpascal}{\rouge{ Ask Pascal }}
\newcommand{\andspace}{\quad \text{ and } \quad}
\newcommand{\unsur}[1]{\frac{1}{#1}}
\newcommand{\omet}[1]{\details{$\bullet \bullet \bullet \bullet $}}
\newcommand{\finpreuve}{\hfill $\square$}
\newcommand{\guillemets}[1]{``#1''}








%%%%%%%%%%%%%%%%%%%%%%%%%%%% SOME MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\florence}[1]{\textcolor{magenta}{#1}}
\newcommand{\pascal}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\blabla}{\textit{blabla ...}}


\newcommand{\muphi}[1]{\mu_\phi\left( #1  \right)}
\newcommand{\muphiseul}{\mu_\phi}
\newcommand{\sigmaphi}[1]{\sigma_\phi\left( #1  \right) }
\newcommand{\sigmaphiseul}{\sigma_\phi}
\newcommand{\sigmaphisq}[1]{\sigma_\phi^2\left( #1  \right)}
\newcommand{\gtheta}[1]{g_\theta( #1 )}
\newcommand{\gthetaseul}{g_\theta}
\newcommand{\getoil}[1]{g^*(#1)}
\newcommand{\getoilseul}{g^*}
\newcommand{\encfunc}[1]{Q_\phi \left( #1  \right)}
\newcommand{\encfuncseul}{Q_\phi}
\newcommand{\qphi}[1]{q_\phi(#1)}
\newcommand{\ptheta}[1]{p_\theta(#1)}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\mse}[1]{\text{MSE}(#1)}
\newcommand{\kmu}{K_\mu}
\newcommand{\ksigma}{K_\sigma}
\newcommand{\ketoil}{K_*}
\newcommand{\ktheta}{K_\theta}
\newcommand{\kphi}{K_\phi}
\newcommand{\leqstar}{\stackrel{(*)}{\leq}}
\newcommand{\muhat}{\mu_{\phi, \theta}}
\newcommand{\muhatn}{\hat{\mu}_{\phi, \theta}}
\newcommand{\otimesn}{^{\otimes n}}
\newcommand{\diam}[1]{\text{diam}(#1)}
\newcommand{\dimetoil}{{d^*}}
\newcommand{\petoil}{p^*}
\newcommand{\tv}[1]{d_{TV}( #1 )}
\newcommand{\tvseul}[1]{d_{TV}}
\newcommand{\ean}{e_a(n, \dimetoil)}
\newcommand{\unvec}{\Vec{1}}
\newcommand{\newf}{\mathcal{E}}
\newcommand{\zetoil}{\wvector}


\newcommand{\zgivenx}{\zvector | \xvector}
\newcommand{\xgivenz}{\xvector | \zvector}
\newcommand{\cdotgivenx}{\cdot | \xvector}
\newcommand{\norme}[1]{\norm{ #1 }}  % maybe I'll want to use ||_2 at the end.
\newcommand{\lossrec}{\loss_\text{rec}^\theta}
\newcommand{\somecitation}{\details{(cite ...)}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%% SOME MACROS APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\qhatn}{\hat{q}_\phi}
\newcommand{\erf}[1]{\text{erf}\left(#1 \right)}
\newcommand{\trace}[1]{\text{Tr} \left( #1 \right)}
\newcommand{\frobnorm}[1]{\norm{#1}_{\text{Fr}}}
\newcommand{\efancy}{\mathcal{E}}
\newcommand{\lrec}{l_\text{rec}^\theta}



